Render-in-the-loop aerial robotics simulator: Case Study on Yield Estimation in Indoor Agriculture

Inspired by recent promising results in sim-to-real transfer in deep learning we built a realistic simulation environment combining a Robot Operating System (ROS)-compatible physics simulator (Gazebo) with Cycles, the realistic production rendering engine from Blender. The proposed simulator pipeline allows us to simulate near-realistic RGB-D images. To showcase the capabilities of the simulator pipeline we propose a case study that focuses on indoor robotic farming. We developed a solution for sweet pepper yield estimation task. Our approach to yield estimation starts with aerial robotics control and trajectory planning, combined with deep learning-based pepper detection, and a clustering approach for counting fruit. The results of this case study show that we can combine real time dynamic simulation with near realistic rendering capabilities to simulate complex robotic systems.

==> content/2mission_planning.tex <==
\section{Mission planning} \label{sec:mission_planning}

To enable the heterogeneous team of robots to work together, we need to establish a mission planning and coordination procedure for these types of systems. Mission planning is a complex problem that is often summarized as two distinct sub-problems, namely the task allocation problem (the question of \emph{who does what?}) and the task scheduling problem (the question of \emph{how to arrange tasks in time?}). 

The tasks we model in this paper fall into the class of problems XD[ST-SR-TA] defined in the taxonomy in \cite{korsahTaxonomy}. These task types require execution by a single robot (SR, single-robot tasks), and robots are allowed to execute only one task at a time (ST, single-task robots). The task allocation and scheduling procedure considers both current and future assignments (TA, time-extended assignment). In terms of complexity, these tasks involve cross-schedule dependencies (XD), where various constraints relate tasks from plans of different robots.

\subsection{Current approaches}

Some of the best known distributed solutions to the multi-robot mission planning problem are auction- and market-based approaches \cite{Otte2017,Nunes2017,Choi2009}. They usually solve the task allocation problem, where robots use bidding mechanisms for simple tasks that they assign to each other. However, the partial ordering between tasks and the tight coupling underlying our cooperative missions are often not considered. More recently, in \cite{Nunes2017,Mitiche2019}, the authors addressed the problem of precedence constraints in iterative auctions for the problem class XD.

On the other side of the spectrum, various optimization-based methods attempt to solve the task planning problem. They range from exact offline solutions \cite{Korsah2011} to heuristic approaches such as evolutionary computation and other AI optimization methods \cite{Mouradian2017,Jevtic2012,Luo2015}. In the former, the problem of class XD[ST-MR-TA] is modeled as an instance of a Mixed-Integer Linear Programming (MILP) problem and solved using offline solvers or known optimization methods. Although the strategy is optimal, it is computationally expensive and lacks reactivity in dynamic environments.

\subsection{Problem definition and modeling}

The mission planning procedure considers a problem where a team of heterogeneous robots $R = \{1,\ldots,m\}$ is available to perform a collection of simple single agent tasks (\emph{actions}) $A = \{1,\ldots,n\}$. A solution to the problem described is a set of time-related actions (\emph{schedule}) for all robots. Formally, the schedule $s_i$ for each robot $i \in R$ is defined as $s_i = \{(a, a^s, a^f)\ \forall a \in S_i\}$, where $S_i$ is the set of actions assigned to robot $i$, and $a^s (a^f)$ are the start (finish) times of action $a$.

Each action $a \in A$ is associated with a couple $(d_a(i), c_a(i)), \forall i \in R$, where $d_a(i)$ represents the duration of action $a$ when executed by robot $i$ and $c_a(i)$ represents the cost of the action. Each robot estimates the duration and cost of a future action based on the current state of the system and its capabilities.

All solutions to the problem must satisfy the \emph{precedence constraints} stated in the mission specification, which are defined as follows. If action $a \in A$ must finish before action $b \in A$ begins, a constraint is generated as $prec(a, b)$. This constraint enforces $a^f < b^s$, where $a^f$ and $b^s$ specify the times at which action $a$ finishes and $b$ begins.

In solving this problem, we model task planning as Multi-Depot Vehicle Routing Problem (MDVRP) with heterogenenous fleet \cite{Salhi2014} and precedence constraints. Essentially, MDVRP is a routing problem for vehicles with limited payloads to pick up or deliver items at different locations. The goal is to find routes for vehicles with the lowest cost without exceeding the vehicle capacity. Given the many similarities between task planning and MDVRP, by modeling the task planning problem as MDVRP, we can apply many optimization techniques already available for this model to our problem. %Moreover, the MDVRP representation generalizes the problem so that the solution can be readily applied to many different domains. %A similar modeling was proposed in \cite{Korsah2011}, where the task planning problem refers to the Dial-a-Ride Problem (DARP), a variant of Vehicle Routing Problem (VRP) with pickup and delivery.

In associating the task planning problem with the MDVRP model, we directly equate the basic VRP concepts with the task planning paradigm. The idea of a depot in MDVRP is directly associated with the initial position of the robot, and the vehicle in MDVRP represents a robot itself. The concept of customer and customer demand relates to actions in task planning and the cost of each action, respectively. Consequently, routes as solutions to VRP problems represent ordered actions in the final robot schedules in the task planning model.

\subsection{Solution approach}

We employ multi-objective optimization using a distributed genetic algorithm with mimetism and knowledge sharing to solve the specified problem. This approach, which uses distributed evolutionary computation methods, can quickly generate near-optimal solutions and therefore work online while achieving good scalability properties. The method we use is inspired by the Coalition-Based Metaheuristic (CBM) algorithm \cite{Meignan2009}, with specific implementation to meet our problem requirements.

The algorithm works very similarly to Genetic Algorithm (GA) in that the solutions in both are represented in terms of chromosomes, which are modified by genetic operators in search of the optimal solution configuration. An important difference is that in CBM, the choice of the operator to apply is not completely stochastic, since this algorithm stores information about its past actions and their potential to obtain solutions that are more likely to lead to better results. Moreover, CBM is a distributed algorithm that runs on multiple agent nodes (in a robotic system, agents are robots). The robots can share their acquired knowledge as well as the best solutions they have found. Therefore, each robot not only learns from its own experience, but can also exhibit mimetic behavior.

Inspired by an evolutionary process, solutions expressed as chromosomes contain genetic material (genotype) that defines each solution. For our problem, this refers to the assignment of actions to different robots and their order within the schedule. Each chromosome is associated with a phenotype that evaluates the genetic material and, in our case, generates schedules for task sequences based on the temporal properties of the tasks (task duration, time of transitioning between tasks).

The algorithm maintains a population of solutions to which it applies various genetic operators. As an evaluation function, we apply a double-rank strategy that scores individuals in the population based on several criteria. Specifically, we use two, makespan of the schedule and the total cumulative cost. In the first part of the evaluation, we use a Pareto ranking procedure \cite{Kalyanmoy2001} that assigns ranks to all solutions based on the non-dominance property (i.e., a solution with a lower rank is clearly superior to solutions with a higher rank regarding all objectives). Therefore, the solutions are stratified into multiple ranks based on their ability to meet the optimization objectives. The second part of the evaluation procedure is the density function, which determines how similar the solution is to other individuals in the population. Finally, the rank and density scores are combined in the fitness of each solution $fitness \in \mathbb{R}_0$.

We chose genetic crossover and mutation from the literature \cite{Pereira2009} as search guiding operators and adapted them to the specifics of our problem. The implemented crossover operator is a version of Best-Cost Route Crossover (BCRC). For mutation, we use the intra-depot and inter-depot swapping operators, as well as single customer rerouting. The details of the individual operators are not included in this paper due to space limitations.

==> content/6conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}


